Scaling physics-informed hard constraints with mixture-of-experts

Imposing known physical constraints, such as conservation laws, during neural network training introduces an inductive bias that can improve accuracy, reliability, convergence, and data efficiency for modeling physical dynamics. While such constraints can be softly imposed via loss function penalties, recent advancements in differentiable physics and optimization improve performance by incorporating PDE-constrained optimization as individual layers in neural networks. This enables a stricter adherence to physical constraints. However, imposing hard constraints significantly increases computational and memory costs, especially for complex dynamical systems. This is because it requires solving an optimization problem over a large number of points in a mesh, representing spatial and temporal discretizations, which greatly increases the complexity of the constraint. To address this challenge, we develop a scalable approach to enforce hard physical constraints using Mixture-of-Experts (MoE), which can be used with any neural network architecture. Our approach imposes the constraint over smaller decomposed domains, each of which is solved by an "expert" through differentiable optimization. During training, each expert independently performs a localized backpropagation step by leveraging the implicit function theorem; the independence of each expert allows for parallelization across multiple GPUs. Compared to standard differentiable optimization, our scalable approach achieves greater accuracy in the neural PDE solver setting for predicting the dynamics of challenging non-linear systems. We also improve training stability and require significantly less computation time during both training and inference stages.

==> problem-setup.tex <==

For the framing - you should only breifly mention the pde in genearlity. You need to spell out how the problem maps to the method. make that link very clearly

at the end you could mention dangers of collapsing + NaNs.


problem setup / framing:

- intro you should describe the pde
    -- put in the form of the pde
    -- things that are more general you can put in a separate section
    -- its expensive to generate numerical solver solns
        -- esp if it is accurate
    -- we need data efficiency 
    -- Talk about how pde error is a better metric (we need better ways to benchmark that doesn't require generating a lot of pde data) - data loss trains to a bad thing
    -- the problem itself is well posed (google for the wiki page) - but the setting for PINNs may not be due to MSE error. If you have too few BCs it may well not be well posed
    -- mention that we have a soft constraint which is known as pinns
    
- problem setup
    -- this is where you talk about the form of the pde
    -- emphasis theres not data in the domain
    -- include details about the training and test dataset (including counts)
    -- setup how many sampled points and difference between MoE and Soft
    -- move the techincal details currently into the problem setup
    -- also include details about the FNO architecture (layers, num modes, batch norm usage etc.)
    -- explicitly talk about how IC \& BC are handled
    -- really to setup our approach but should setup the comparison
- problem details
    -- talk about the optimization problem
    -- here define the LM objective function
    -- put tolerance + iterations here
- Results sections
    -- point to the figs to showcase the predictions
    -- See section for core figs
    -- PDE residual plots + difference plots can go in the appendix.
    -- Also include loss plots here on validation set (soft & hard constraint should be on the same figure).
    -- Could also include L2 relative error plot
    -- Table to summarize results (final losses + you can add timing results)
    -- The graph should also include a dotted line for the numerical solver for PDE residual (esp if that number is higher than the MoE results) avg over many points
    -- Shows that we can go below the numerical solver error or are on par
    -- For timings:
        -- Inference time per PDE + total training time
        -- Need to make it clear what per PDE means
        -- Use total training time
        -- Just make it clear how the timings are computed

- Data sparsity
    -- To show we need less data than a soft constraint
    -- This is the closest to replacing a numerical solver
    -- Dashed line for PC-MoE \& no data. then use multiple runs of the soft constraint for the lines. 
    -- Dashed line would be u (best MoE model with no data)
    -- have a second y axis for time that shows how long it takes to generate that much data.
    -- Two versions - one with just time to generate data and one with time generate and train
        -- for the hard constraint timing - just ignore for now and see how it look
    -- Also include the purely data driven approach errors with increasing amounts of training data.
    -- So the final plot should include 1. purely data driven 2. soft constraint 3. the pc-moe


Colormaps: Orange \& blue are good contrastive colors

Use the python package SciencePlots for figures like loss \& timing. 

==> s0-todo.tex <==
\draft{\section*{TODO}

High Level Notes

\begin{itemize}
    \item We might want to pitch this as a physics informed hard constraint - might be more appealing to the PINNs people. Example of piggy-backing off of the PINNs name: PINNs hard constraint paper.
    \item We are instead showing that we scale physics constraints.
    \item potentially include a schematic of different types of domain decomposition possible with MoE
\end{itemize}

}
